Merging Multiparty Protocols in Multiparty Choreographies

Choreography-based programming is a powerful paradigm for defining communication-based systems from a global viewpoint. A choreography can be checked against multiparty protocol specifications, given as behavioural types, that may be instantiated indefinitely at runtime. Each protocol instance is started with a synchronisation among the involved peers. We analyse a simple transformation from a choreography with a possibly unbounded number of protocol instantiations to a choreography instantiating a single protocol, which is the merge of the original ones. This gives an effective methodology for obtaining new protocols by composing existing ones. Moreover, by removing all synchronisations required for starting protocol instances, our transformation reduces the number of communications and resources needed to execute a choreography.

==> eptcsdata.tex <==
\providecommand{\firstpage}{21}
\providecommand{\publicationstatus}{S. J. Gay and P. H. Kelly (Eds.): Programming Language Approaches to\\
Concurrency- and Communication-cEntric Software (PLACES 2012)\\
EPTCS 109, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.109.4}{10.4204/EPTCS.109.4}}

